Multi-task Heterogeneous Graph Learning on Electronic Health Records

Learning electronic health records (EHRs) has received emerging attention because of its capability to facilitate accurate medical diagnosis. Since the EHRs contain enriched information specifying complex interactions between entities, modeling EHRs with graphs is shown to be effective in practice. The EHRs, however, present a great degree of heterogeneity, sparsity, and complexity, which hamper the performance of most of the models applied to them. Moreover, existing approaches modeling EHRs often focus on learning the representations for a single task, overlooking the multi-task nature of EHR analysis problems and resulting in limited generalizability across different tasks. In view of these limitations, we propose a novel framework for EHR modeling, namely MulT-EHR (Multi-Task EHR), which leverages a heterogeneous graph to mine the complex relations and model the heterogeneity in the EHRs. To mitigate the large degree of noise, we introduce a denoising module based on the causal inference framework to adjust for severe confounding effects and reduce noise in the EHR data. Additionally, since our model adopts a single graph neural network for simultaneous multi-task prediction, we design a multi-task learning module to leverage the inter-task knowledge to regularize the training process. Extensive empirical studies on MIMIC-III and MIMIC-IV datasets validate that the proposed method consistently outperforms the state-of-the-art designs in four popular EHR analysis tasks -- drug recommendation, and predictions of the length of stay, mortality, and readmission. Thorough ablation studies demonstrate the robustness of our method upon variations to key components and hyperparameters.

==> chatgpt_outputs/multi-task-learning.tex <==
Could you explain how the cross-task variance regularization term works?

The cross-task variance regularization term is a penalty term that is added to the loss function during training to encourage the model to learn representations that are invariant across tasks. The intuition behind this is that if the model learns to represent the input data in a way that is consistent across different tasks, then it should be better able to generalize to new tasks or data that it has not seen before.

The cross-task variance term is computed by comparing the predicted outputs of the current task with the predicted outputs of all other tasks. Specifically, for a given task, the regularization term is defined as the L2 norm of the difference between the predicted outputs of the current task and the predicted outputs of all other tasks. The intuition behind this is that if the predicted outputs of the current task are very different from the predicted outputs of other tasks, then the model is likely overfitting to the current task and not learning generalizable representations.

The regularization term is then added to the loss for the current task, with a weight specified by the ct_var_weight parameter in the config_gnn dictionary. The weight controls the strength of the regularization term relative to the main loss term, and can be tuned through experimentation to find the optimal balance between encouraging invariance across tasks and preserving task-specific information.

By minimizing the cross-task variance regularization term along with the main loss term, the model is encouraged to learn representations that are both task-specific and invariant across tasks, leading to better generalization performance.


